Learning to Blame: Localizing Novice Type Errors with Data-Driven Diagnosis

Localizing type errors is challenging in languages with global type inference, as the type checker must make assumptions about what the programmer intended to do. We introduce Nate, a data-driven approach to error localization based on supervised learning. Nate analyzes a large corpus of training data -- pairs of ill-typed programs and their "fixed" versions -- to automatically learn a model of where the error is most likely to be found. Given a new ill-typed program, Nate executes the model to generate a list of potential blame assignments ranked by likelihood. We evaluate Nate by comparing its precision to the state of the art on a set of over 5,000 ill-typed OCaml programs drawn from two instances of an introductory programming course. We show that when the top-ranked blame assignment is considered, Nate's data-driven model is able to correctly predict the exact sub-expression that should be changed 72% of the time, 28 points higher than OCaml and 16 points higher than the state-of-the-art SHErrLoc tool. Furthermore, Nate's accuracy surpasses 85% when we consider the top two locations and reaches 91% if we consider the top three.

==> evaluation-accuracy-recall-graph.tex <==

% colors from http://colorbrewer2.org/?type=sequential&scheme=Blues&n=3
\definecolor{blue1}{HTML}{DEEBF7}
\definecolor{blue2}{HTML}{9ECAE1}
\definecolor{blue3}{HTML}{3182BD}

\definecolor{green1}{HTML}{e5f5e0}
\definecolor{green2}{HTML}{a1d99b}
\definecolor{green3}{HTML}{31a354}

% \begin{figure}[ht]
% \centering
% \begin{tikzpicture}
% \begin{axis}[
%   % ybar stacked,
%   width=12cm,
%   height=8cm,
%   title={Impact of Feature Set on Accuracy},
%   ylabel={Accuracy},
%   %ymin=0.2,
%   ymax=1,
%   yticklabel={\pgfmathparse{\tick*100}\pgfmathprintnumber{\pgfmathresult}\,\%},
%   ytick style={draw=none},
%   ymajorgrids = true,
%   symbolic x coords={op+type+size, op+context+type+size, op+context-has+type+size, op+context-count+type+size},
%   % enlarge x limits=0.25,
%   xtick=data,
%   xtick style={draw=none},
%   xticklabels={Type, Context-Is, Context-Has, Context-Count},
%   x tick label style={rotate=45},
%   reverse legend,
%   transpose legend,
%   legend style={legend pos = outer north east, legend columns=4},
% ]
% % \addplot[draw=black, fill=blue1] table[x=tool, y=top-1] {\HiddenBench};
% % \addplot[draw=black, fill=blue2] table[x=tool, y expr=\thisrow{top-2} - \thisrow{top-1}] {\HiddenBench};
% % \addplot[draw=black, fill=blue3] table[x=tool, y expr=\thisrow{top-3} - \thisrow{top-2}] {\HiddenBench};

% \addplot[mark options={fill=blue1, scale=1.5}, mark=square*]
%   table[x=features, y=top-1] {\FeatureHiddenFHBench};
% \addplot[mark options={fill=blue2, scale=1.5}, mark=square*]
%   table[x=features, y=top-2] {\FeatureHiddenFHBench};
% \addplot[mark options={fill=blue3, scale=1.5}, mark=square*]
%   table[x=features, y=top-3] {\FeatureHiddenFHBench};
% \addlegendentry{Top-1}
% \addlegendentry{Top-2}
% \addlegendentry{Top-3}
% \addlegendimage{empty legend}
% \addlegendentry{\hiddenFH}

% \addplot[mark options={fill=blue1, scale=1.5}, mark=*]
%   table[x=features, y=top-1] {\FeatureLinearBench};
% \addplot[mark options={fill=blue2, scale=1.5}, mark=*]
%   table[x=features, y=top-2] {\FeatureLinearBench};
% \addplot[mark options={fill=blue3, scale=1.5}, mark=*]
%   table[x=features, y=top-3] {\FeatureLinearBench};
% \addlegendentry{Top-1}
% \addlegendentry{Top-2}
% \addlegendentry{Top-3}
% \addlegendimage{empty legend}
% \addlegendentry{\linear}

% \end{axis}
% \end{tikzpicture}
% \caption{reuslts!}
% \label{fig:results}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \begin{tikzpicture}
% \begin{axis}[
%   ybar stacked,
%   width=12cm,
%   height=8cm,
%   title={Impact of Hidden Layer Size on Accuracy},
%   ylabel={Accuracy},
%   bar width=20pt,
%   %ymin=0.2,
%   ymax=1,
%   yticklabel={\pgfmathparse{\tick*100}\pgfmathprintnumber{\pgfmathresult}\,\%},
%   ytick style={draw=none},
%   ymajorgrids = true,
%   symbolic x coords={op+type+size/hidden-10, op+type+size/hidden-25, op+type+size/hidden-50,
%                      op+type+size/hidden-100, op+type+size/hidden-250, op+type+size/hidden-500},
%   % enlarge x limits=0.25,
%   xtick=data,
%   xtick style={draw=none},
%   xticklabels={\hiddenT, \hiddenTF, \hiddenF, \hiddenH, \hiddenTHF, \hiddenFH},
%   x tick label style={rotate=45},
%   reverse legend,
%   legend style={legend pos = north west},
% ]
% \addplot[draw=black, fill=blue1] table[x=tool, y=top-1] {\HiddenBench};
% \addplot[draw=black, fill=blue2] table[x=tool, y expr=\thisrow{top-2} - \thisrow{top-1}] {\HiddenBench};
% \addplot[draw=black, fill=blue3] table[x=tool, y expr=\thisrow{top-3} - \thisrow{top-2}] {\HiddenBench};
% % \addplot[draw=black, fill=blue1] table[x=tool, y=top-1] {\HiddenBench};
% % \addplot[draw=black, fill=blue2] table[x=tool, y=top-2] {\HiddenBench};
% % \addplot[draw=black, fill=blue3] table[x=tool, y=top-3] {\HiddenBench};
% \legend{Top-1, Top-2, Top-3}
% \end{axis}
% \end{tikzpicture}
% \caption{reuslts!}
% \label{fig:results}
% \end{figure}

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
  ybar stacked,
  width=\linewidth,
  height=8cm,
  title={Accuracy of Type Error Localization Techniques},
  ylabel={Accuracy},
  bar width=0.5cm,
  ymin=0.2,
  ymax=1,
  ytick={0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0},
  yticklabel={\pgfmathparse{\tick*100}\pgfmathprintnumber{\pgfmathresult}\,\%},
  ytick style={draw=none},
  ymajorgrids = true,
  symbolic x coords={baseline, ocaml, spacer1, mycroft, sherrloc, spacer2,
                     op+context+type+size/linear,
                     op+context+type+size/decision-tree,
                     op+context+type+size/random-forest,
                     op+context+type+size/hidden-10,
                     op+context+type+size/hidden-500},
  % enlarge x limits=0.5,
  xtick=data,
  xtick style={draw=none},
  xticklabels={\random, \ocaml, \mycroft, \sherrloc,
               \linear, \dectree, \forest, \hiddenT, \hiddenFH},
  x tick label style={rotate=45, anchor=north east},
  reverse legend,
  transpose legend,
  legend style={legend pos = north west, legend columns=5},
]

% ES: NOTE: ORDER OF PLOTS/LEGEND ENTRIES MATTERS
\addplot+[stack plots=false, draw=black, fill=none, thick, bar shift=.25cm] table[x=tool, y=recall] {\FallBench};
\addlegendentry{Recall}
\addplot[draw=black, fill=green1, bar shift=.25cm] table[x=tool, y=top-1] {\FallBench};
\addlegendentry{Top-1}
\addplot[draw=black, fill=green2, bar shift=.25cm] table[x=tool, y expr=\thisrow{top-2} - \thisrow{top-1}] {\FallBench};
\addlegendentry{Top-2}
\addplot[draw=black, fill=green3, bar shift=.25cm] table[x=tool, y expr=\thisrow{top-3} - \thisrow{top-2}] {\FallBench};
\addlegendentry{Top-3}
\addlegendimage{empty legend}
\addlegendentry{\FALL}

\resetstackedplots

\addplot+[stack plots=false, draw=black, fill=none, thick, bar shift=-.25cm] table[x=tool, y=recall] {\SpringBench};
\addlegendentry{Recall}
\addplot[draw=black, fill=blue1, bar shift=-.25cm] table[x=tool, y=top-1] {\SpringBench};
\addlegendentry{Top-1}
\addplot[draw=black, fill=blue2, bar shift=-.25cm] table[x=tool, y expr=\thisrow{top-2} - \thisrow{top-1}] {\SpringBench};
\addlegendentry{Top-2}
\addplot[draw=black, fill=blue3, bar shift=-.25cm] table[x=tool, y expr=\thisrow{top-3} - \thisrow{top-2}] {\SpringBench};
\addlegendentry{Top-3}
\addlegendimage{empty legend}
\addlegendentry{\SPRING}


%\legend{Top-1, Top-2, Top-3}
\end{axis}
\end{tikzpicture}
\caption{
  %
  Results of our comparison of type error localization
  techniques.
  %
  We evaluate all techniques separately on two cohorts of
  students from different instances of an undergraduate
  Programming Languages course.
  %
  Our classifiers were trained on one cohort and evaluated on the other.
  %
  All of our classifiers outperform the state-of-the-art techniques
  \mycroft and \sherrloc by a 10--15\% margin in Top-1 accuracy (with
  the exception of \linear which is only slightly better than \sherrloc).
%
}
\label{fig:accuracy-results}
\end{figure}


==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Type systems are one of the most widely-used techniques for program
verification. A type checker only accepts a program if it can
\emph{prove} the absence of an entire class of bugs.
%
Typed functional languages like \ocaml and \haskell are equipped with
particularly powerful type checkers that can operate without a single
annotation, alleviating a prime concern with verification techniques.
%
Yet this power comes with a cost: type annotations signify the
programmer's \emph{intent}, without them the checker must
make assumptions about what the programmer intended to do.
%
This results in the common phenomenon of type errors being reported far
from their source, an annoyance to veterans of the type system, but a
significant hurdle for novices \citep{Wand1986-nw,Joosten1993-yx}.

\begin{figure}[ht]
\begin{minipage}{0.45\linewidth}
\begin{ecode}
  let rec sumList xs =
    match xs with
    | []   -> (*@\hlTree{\hlSherrloc{[]}}@*)
    | h::t -> h (*@\hlTree{+}@*) (*@\hlFix{sumList t}@*)
\end{ecode}
\end{minipage}
\begin{minipage}{0.49\linewidth}
\begin{verbatim}
File "sumList.ml", line 4, characters 16-25:
  This expression has type 'a list
  but an expression was expected of type int
\end{verbatim}
\end{minipage}
\caption{(left) An ill-typed \ocaml program that should sum the elements of a
  list, with highlights indicating three possible blame assignments based on:
  %
  (1) the \hlFix{\ocaml} compiler;
  %
  (2) the \hlSherrloc{fix} made by the programmer; and
  %
  (3) \hlTree{minimizing} the number of edits required.
  % The \underline{underlined} expressions are equally valid
  % locations to blame. The expression blamed by the \ocaml compiler
  % is in \textbf{bold}.
  %
  % FIXME: This bolding is ambiguous, because ``let rec'', ``match'' and
  % ``with'' are also bolded (by \\ecode)! You need to find another way to
  % highlight what ocaml is yelling about.
  %
  (right) The error reported by \ocaml.}
\label{fig:sumList}
\end{figure}
%
Consider the |sumList| program in \autoref{fig:sumList}, written by a
student in an undergraduate Programming Languages course.
%
The program is meant to sum the integers in a list, but the student has
accidentally given the empty list as the base case, rather than 0.
%
The \ocaml compiler collects typing constraints as it traverses the
program, and reports an error the moment it finds an inconsistent
constraint.
%
In this case it blames the recursive call to |sumList|, complaining that
|sumList| returns a |list| where an |int| was expected by the |+|
operator.
%
Note that this blame is inconsistent with the programmer's intention and
may not be helpful debugging information to a novice.

Recent work on type error \emph{localization}
%
\citep[\eg][]{Zhang2014-lv,Loncaric2016-uk,Pavlinovic2014-mr},
%
determining which expression(s) to blame for the error,
frames localization as an optimization problem, seeking a set of
expressions to blame that minimize some cost function (\eg the number of
constraints in the blame set, or the ratio of ``good'' paths through the
constraint graph to ``bad'' paths).
%
However, even these techniques fail to distinguish between the two
underlined expressions in \autoref{fig:sumList}, it would be equally
valid to blame \emph{either} of them alone.
%
The |[]| on line 3 could be changed to |0|, or the |+| on line 4 could
be changed to either |@| (list append) or |::|, all of which would give
type-correct programs.
%
Thus, these state-of-the-art techniques are forced to either blame
\emph{both} locations, or choose one \emph{arbitrarily}.

It may appear obvious to the reader that |[]| is the correct expression
to blame, but how is the type checker to know that?
%
Our solution is to \emph{learn} how to localize type errors by observing
a large set of (novice) errors and their \emph{subsequent fixes}.
%
We accomplish this via three concrete contributions.

\paragraph{\textbf{(1) A Dataset of Novice \ocaml Programs}}
Our first contribution is a large dataset of novice \ocaml programs,
including, but not limited to, \emph{ill-typed} programs.
%
We used an instrumented version of the \ocaml compiler to collect
student interactions over two instances of an undergraduate Programming
Languages course at
%
\begin{anonsuppress}
UC San Diego (IRB \#140608).
\end{anonsuppress}
\begin{noanonsuppress}
AUTHOR's INSTITUTION (IRB HIDDEN).
\end{noanonsuppress}
%
The data consist of a time-series of programs submitted to the \ocaml
compiler, from which we extracted a set of \emph{ill-typed} programs
and their \emph{subsequent fixes}.
%
Our dataset comprises over 4,500 such pairs of programs, and many more
programs that are either well-typed or lack a corresponding fix.
%
The entire dataset (both the raw time-series and our extracted pairs of
ill-typed programs and fixes) is available at
%
\begin{anonsuppress}
\ES{TODO: finally post the data somehwere..}.
\end{anonsuppress}
\begin{noanonsuppress}
HIDDEN FOR DOUBLE-BLIND REVIEW.
\end{noanonsuppress}
%

\paragraph{\textbf{(2) Data-Driven Diagnosis of Type Errors}}
Our second contribution is a \emph{data-driven} technique for localizing
type errors (\autoref{sec:learning}).
%
We use machine learning techniques to train a set of classifiers that can
predict, given an ill-typed program, which expressions should be changed
for the program to type check.
%
Our classifiers can be trained on a relatively small set of programs
(\ie a single course's worth). 
% WRW notes that we say this below in contribution (3), which is only three
% sentences away, so to a first-time reader it sounds like we are
% double-counting:
%
% and outperform the state of the art by
% 15--30\% in blame accuracy.
%
The key technical challenge that we tackle is defining a suitable
interface between the type checker and the classifier, specifically
\emph{embedding} programs as feature vectors and presenting the
classifier's predictions to the user.

\paragraph{\textbf{(3) A Large-Scale Evaluation of Type Error Localization}}
Our third contribution is an evaluation of our classifiers and the
state-of-the-art techniques on our suite of over 4,500 student programs
(\autoref{sec:evaluation}), the largest evaluation of type error
localization techniques we are aware of.
%
We judge the correctness of a localization by comparing it to the
student's eventual fix and find that our classifiers are 15--30\% more
accurate than the state of the art.
%
We also examine which features contribute the most to our
classifiers' predictions, and endeavor to \emph{explain} specific
predictions that our classifiers get right (and wrong).

Overall, our results show that data-driven diagnosis is a practical
technique for localizing type errors by learning from past mistakes.
%
% We believe, furthermore, that with the right set of features our
% approach could be applied to other domains where there are multiple,
% equally valid explanations for an error.
% \ES{this sounds really dumb... need better phrasing}

% \begin{enumerate}
% \item An large-scale evaluation of state-of-the-art type error
%   localization techniques on over 4,500 student programs.
%   %
%   We collected a time-series of \ocaml programs from our students, and
%   use their subsequent \emph{fixes} to ill-typed programs as
%   \emph{oracles} for the location of the error.
%   %
%   This is the most extensive evaluation of the accuracy of type error
%   localization techniques that we are aware of.
%   % based not on expert \emph{opinion}, but
%   % on the eventual \emph{fix} implemented by a novice user.
%   %
%   % \ES{need to explain \emph{why} this is superior..}
% \item A machine learning approach to \emph{modeling} (novice) type
%   errors that can outperform the state-of-the-art by 15--30\% in
%   localizing errors.
%   %
%   Our classifiers can be trained on a relatively small amount of data --- we
%   used a single class of around 50 students --- and appear to
%   generalize to other instances of the same class.
%   %
%   \ES{and hopefully completely separate classes!}
%   %
%   In contrast to many approaches to \emph{fault localization} from the
%   software engineering community, our model does not use any linguistic
%   modeling techniques, \eg \emph{n-grams} over the token stream; rather,
%   it relies entirely on features of the abstract syntax tree and a
%   partial typing derivation.
%   %
%   \ES{if there's time, investigate adding Wes' n-gram model}
% \end{enumerate}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> scratch.tex <==


